Age-Appropriate Robot Design: In-The-Wild Child-Robot Interaction Studies of Perseverance Styles and Robot's Unexpected Behavior

As child-robot interactions become more and more common in daily life environment, it is important to examine how robot's errors influence children's behavior. We explored how a robot's unexpected behaviors affect child-robot interactions during two workshops on active reading: one in a modern art museum and one in a school. We observed the behavior and attitudes of 42 children from three age groups: 6-7 years, 8-10 years, and 10-12 years. Through our observations, we identified six different types of surprising robot behaviors: personality, movement malfunctions, inconsistent behavior, mispronunciation, delays, and freezing. Using a qualitative analysis, we examined how children responded to each type of behavior, and we observed similarities and differences between the age groups. Based on our findings, we propose guidelines for designing age-appropriate learning interactions with social robots.

==> tables.tex <==
% children 6-7 yrs
\begin{longtable}{ |p{3.5cm}|p{5cm}|}
 \hline
 \multicolumn{2}{|c|}{Unexpected behaviors: children (6-7 yrs)\\ %observed during the study} \\
 %\multicolumn{2}{|c|}{Children of 6-7 years old}\\
\hline
Category of behavior&Event\\
\hline
Robot's personality&Robot presents information about its close relations, by saying that it has friends or that it doesn’t remember it’s parents.\\
\cline{2-2}
&Robot presents information about its food preferences by saying that it eats disks for supper and batteries for breakfast. \\
\cline{2-2}
&Robot presents information about its lack of knowledge by asking children questions.\\
\cline{2-2}
&Robot presents information about its origin by saying that it’s from Japan. \\

\hline
Movement limitations&Robot can’t walk multiple times during the interaction. \\
\cline{2-2}
&Robot can’t move its hands when asked to. \\
\cline{2-2}
&Robot can’t turn around and asks a facilitator to turn it around multiple times during the interaction.\\

\hline
Inconsistent behaviors
&Robot reacts to the facilitator’s invitation to take pictures by saying “Pictures”, which to children sounds like “Kittens”. \\

\hline
Mispronunciation& Robot reacts to the facilitator’s invitation to take pictures by saying “Pictures”, which to children sounds like “Kittens”.\\

\hline
Delays& Robot provides answers after relatively long time from the questions being asked (relating to human answering questions). \\

\hline
Freezing& Robot freezes multiple times during the interaction and doesn’t move or speak.\\
\cline{2-2}
&Robot freezes multiple times during the interaction and doesn’t respond to children’s or facilitator’s questions.\\
\hline
\end{longtable}

% children 8-10 yrs
\begin{longtable}{|p{3.5cm}|p{5cm}|}
\hline
\multicolumn{2}{|c|}{Unexpected behaviors: Children (8-10 yrs)\\% children observed during the study} \\
% \multicolumn{2}{|c|}{Children of 8-10 years old}\\
\hline
Category of behavior&Event\\
\hline
Robot's personality&Robot presents information about it's math abilities, correctly solving a math problem "what is 2+2".\\
\cline{2-2}
&Robot presents information about it's math abilities, correctly solving a math problem "what is 5x5".\\
\cline{2-2}
&Robot presents information about it's math abilities, by correctly counting from 1 to 10.\\
\cline{2-2}
&Robot presents information about it's language abilities by saying "Si" in Spanish.\\
\cline{2-2}
&Robot presents information about it's language abilities by saying "Konnichi'wa" in Japanese.\\
\cline{2-2}
&Robot presents information about it's language abilities by saying "Spasiba" in Russian.\\
\hline
Movement limitations&Robot can't walk more than few steps. 
\cline{2-2}
&Robot is slow in moving and changing poses, e.g. sitting or standing up. 
\cline{2-2}
&Robot can't move it's hand to shake hands with children. 
\cline{2-2}
&Robot can't move it's hand to do a high-five with children. 
\cline{2-2}
&Robot can't jump. 
\cline{2-2}
&Robot can't dance certain dances. 
\hline
Inconsistent behaviors&Robot plays growling sound while playing a character in a story. 
\cline{2-2}
&Robot plays ovation sound while playing a character in a story. 
\cline{2-2}
&Robot plays machine sound while playing a character in a story. 
\cline{2-2}
&Robot plays automatic information about low battery while playing a character in a story.
\hline
Mispronunciation&Robot says 'I do' that sounds like 'I don't'.
\cline{2-2}
&Robot says 'N' that sounds like 'M'.
\hline
Delays&Robot reads a story by reading few words at a time and stopping for few seconds. 
\hline
Freezing&Robot freezes multiple times during the interaction and doesn’t respond to children's questions and requirements. 
\hline
\end{longtable}

% children 10-12 yrs
\begin{longtable}{|p{3.5cm}|p{5cm}|}
 \hline
 \multicolumn{2}{|c|}{Unexpected behaviors: Children (10-12 yrs)\\% observed during the study} \\
 %\multicolumn{2}{|c|}{Children of 10-12 years old}\\
\hline
Category of behavior&Event\\
\hline
 Robot's personality&Robot presents information about it’s age, by saying “I’m six years old.”\\
\cline{2-2}
 &Robot presents information about it’s food preferences, by saying that it likes vegan hotdogs and that it’s vegan. \\
\cline{2-2}
 &Robot presents its knowledge by answering children’s questions.\\
 \cline{2-2}
 & Robot presents information about its belonging by saying “I am an owner to myself.”\\
\cline{2-2}
 &Robot presents information about its origin by saying that it’s from Japan.\\
 \cline{2-2}
 &Robot presents information about its gender by saying that it’s a boy.\\
 \hline
 Movement limitations&Robot can’t walk while being invited to meet the children at the beginning of the interaction and has to be carried by the facilitator. \\
 \cline{2-2}
 &Robot can’t turn around and asks a facilitator to turn it around multiple times during the interaction. \\ 
 \cline{2-2}
 &Robot can’t dance a certain dance while being asked to.\\
 \cline{2-2}
 &Robot can’t run while being asked to.\\
 \cline{2-2}
 & Robot can’t jump while being asked to.\\
 \hline
 Inconsistent behaviors&Robot tells children it knows German language and later it tells children it doesn’t know German language.\\
 \cline{2-2}
 & Robot is correctly guessing child’s pose during the game of charades while having it's face pointed in opposite direction than the child.\\
 \cline{2-2}
 &Robot tells children that it’s vegan and later on nods while a child asks it if it eats meet.\\
 \cline{2-2}
 & Robot says it will dance and doesn’t dance.\\
 \hline
 Mispronunciation&Robot says “I will in a minoote” instead of “a minute”.\\
 \cline{2-2}
 &Robot reacts to a question “Why are you vegan?” by saying “I love animals”, which to children sounds as “I love lemons”.\\
 \hline
 Delays&Robot provides answers after relatively long time from the questions being asked (relating to human answering questions).\\
 \cline{2-2}
 &Robot answers a previous question by saying “yes” while a child asks a new one: “Do you eat meat?” \\
 \cline{2-2}
 &Robot answers a previous question by nodding while a child asks a new one: “Can you take over the word?"\\
 \hline
 Freezing&Robot freezes multiple times during the interaction and doesn’t move or speak.\\
 \cline{2-2}
&Robot freezes multiple times during the interaction and doesn’t respond to children’s or facilitator’s questions.\\
\hline
\end{longtable}

